MM-VID: Advancing Video Understanding with GPT-4V(ision)

We present MM-VID, an integrated system that harnesses the capabilities of GPT-4V, combined with specialized tools in vision, audio, and speech, to facilitate advanced video understanding. MM-VID is designed to address the challenges posed by long-form videos and intricate tasks such as reasoning within hour-long content and grasping storylines spanning multiple episodes. MM-VID uses a video-to-script generation with GPT-4V to transcribe multimodal elements into a long textual script. The generated script details character movements, actions, expressions, and dialogues, paving the way for large language models (LLMs) to achieve video understanding. This enables advanced capabilities, including audio description, character identification, and multimodal high-level comprehension. Experimental results demonstrate the effectiveness of MM-VID in handling distinct video genres with various video lengths. Additionally, we showcase its potential when applied to interactive environments, such as video games and graphic user interfaces.

==> 04-analysis.tex <==
% \section{\modelname~System Paradigm}
% \modelname~is related to previous explorations~\cite{tsimpoukelli2021multimodal,alayrac2022flamingo,li2023blip,huang2023language,driess2023palme,gpt4,yang2022empirical,zeng2022socratic,wanglanguage,hu2022promptcap} on extending LLMs with vision capabilities. We discuss the pros and cons of \modelname's system paradigm with additional analyses and case studies.

% \subsection{Vision Module}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% One difference is that \modelname~utilizes selected specialized vision experts to perceive visual signals, in contrast to the standard approach of utilizing a single, general-purpose vision module.

% \noindent\textbf{Specialized Vision Experts.} Selecting proper specialized vision experts may provide more informative signals for specific vision problems. Examples of pose estimation, counting+math reasoning, or document understanding.

% \noindent\textbf{Collaboration of Vision Experts.} The synergetic collaboration of multiple vision experts could further boost \modelname’s vision capability.

% \noindent\textbf{Limitations.}
% Errors caused by failing to invoke correct vision experts.

% \subsection{Module Communication}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Modules in \modelname~communicate with text prompts, different from previous studies~\cite{tsimpoukelli2021multimodal,alayrac2022flamingo,li2023blip,huang2023language,driess2023palme} that more closely bind vision and language modules via joint finetuning.

% \noindent\textbf{Capability comparison with PaLM-E.}
% Despite the great flexibility and being easy to expand, it is unclear whether communicating with prompts will lose any capabilities achieved by joint finetuning. As shown in Figure~\ref{fig:palme1}-\ref{fig:palme4}, we conduct a comparison with the core capability illustrated by a recent study PaLM-E~\cite{driess2023palme}, and empirically show that text prompts are effective in achieving such capability. We illustrate the complete chain-of-thoughts reasoning and action procedures in Figures~\ref{fig:palme-cot-3}-\ref{fig:palme-cot-5}.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=.8\textwidth]{figure/palme.pdf}
% \caption{Comparison of \modelname~with PaLM-E~\cite{driess2023palme} on illustrated capabilities. We empirically show that text prompts are effective as expensive joint fine-tuning in solving complicated vision problems. 
% \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/EUIuISjAEh5GoZd5ASdC6IEBzG0gwqByA97FOIO3kLlpcQ?e=1hzDaJ}
% %\url{https://docs.google.com/drawings/d/1YRKqzQ4m9grR0sUg1OPf2ncP8ddYK_EoduEixJ1kbcU/edit?usp=sharing}
% 	}
% \label{fig:palme}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[width=.9\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme_compare_1.pdf}
% \caption{Comparison of \modelname~with PaLM-E~\cite{driess2023palme} on illustrated capabilities. We empirically show that text prompts are effective as expensive joint fine-tuning in solving complicated vision problems. \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/Edfi-ft0snZPlFHtMFRuVH4BwrwDmIa3tkg38dxYLsxOGA?e=DN6mdm}
% 	}
% \label{fig:palme1}
% \end{figure*}
% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[width=.9\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme_compare_2.pdf}
% \caption{Comparison of \modelname~with PaLM-E~\cite{driess2023palme} on illustrated capabilities. We empirically show that text prompts are effective as expensive joint fine-tuning in solving complicated vision problems. \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/Edfi-ft0snZPlFHtMFRuVH4BwrwDmIa3tkg38dxYLsxOGA?e=DN6mdm}
% 	}
% \label{fig:palme2}
% \end{figure*}
% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[width=.9\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme_compare_3.pdf}
% \caption{Comparison of \modelname~with PaLM-E~\cite{driess2023palme} on illustrated capabilities. We empirically show that text prompts are effective as expensive joint fine-tuning in solving complicated vision problems. \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/Edfi-ft0snZPlFHtMFRuVH4BwrwDmIa3tkg38dxYLsxOGA?e=DN6mdm}
% 	}
% \label{fig:palme3}
% \end{figure*}
% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[width=.9\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme_compare_4.pdf}
% \caption{Comparison of \modelname~with PaLM-E~\cite{driess2023palme} on illustrated capabilities. We empirically show that text prompts are effective as expensive joint fine-tuning in solving complicated vision problems. \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/Edfi-ft0snZPlFHtMFRuVH4BwrwDmIa3tkg38dxYLsxOGA?e=DN6mdm}
% 	}
% \label{fig:palme4}
% \end{figure*}
% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[width=.7\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme_compare_5.pdf}
% \caption{Comparison of \modelname~with PaLM-E~\cite{driess2023palme} on illustrated capabilities. We empirically show that text prompts are effective as expensive joint fine-tuning in solving complicated vision problems. \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/EZZsbmwyGWJFjVXZDS26DKABsLAv0PlBRvW321kRhLWxwg?e=dHuCle}
% 	}
% \label{fig:palme5}
% \end{figure*}

% \noindent\textbf{Flexible Module Update and Customization.}
% Example of module update, or adding own module like the spatial relationship logic.


% Moreover, \modelname's system paradigm allows the synergetic collaboration of LLMs and vision experts. \modelname's flexibility allows the easy upgrade of module components, either language model or vision experts, to yield a stronger system. For example, we can add or refine a specific vision expert to address certain problems observed in the solution chain, such as failing to recognize a certain object. In contrast, it is more complicated to tweak the jointly finetuned, general-purpose vision module for solving a specific weakness without hurting its original capabilities.

% \noindent\textbf{Limitations.}
% Some cases still can not solve? 

% \subsection{Limitations}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% maybe merge into the upper two sub-section?


% \begin{figure*}[t]
% \centering
% \vspace{-24mm}
% \includegraphics[height=1.15\textheight]{iccv2023AuthorKit/figure/mmreact-unfolded-1.pdf}
% \vspace{-14mm}
% \caption{Unfolded multimodal reasoning and action steps for the input image, and the user question is ``How many championship rings did the player on the left win in his career?'' % \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/EYmEmA2AKJFCoUt2vZtY_1EB5zPERmgT7zU-kR7EMls-0g?e=ECYFyu}
% 	}
% \label{fig:mmreact-unfolded-1}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[height=1.35\textheight]{iccv2023AuthorKit/figure/mmreact-unfolded-2.pdf}
% \vspace{-65mm}
% \caption{Unfolded multimodal reasoning and action steps for the input image, and the user question is ``I am getting just two custom pizza for me and my friend. How much
% should I pay in total?'' % \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/EYmEmA2AKJFCoUt2vZtY_1EB5zPERmgT7zU-kR7EMls-0g?e=ECYFyu}
% 	}
% \label{fig:mmreact-unfolded-2}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[height=1.2\textheight]{iccv2023AuthorKit/figure/mmreact-unfolded-3.pdf}
% \vspace{-30mm}
% \caption{Unfolded multimodal reasoning and action steps for the input image, and the user question is ``Where is the coffee pot in the second image?'' % \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/EYmEmA2AKJFCoUt2vZtY_1EB5zPERmgT7zU-kR7EMls-0g?e=ECYFyu}
% 	}
% \label{fig:mmreact-unfolded-3}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \vspace{-20mm}
% \includegraphics[height=1.2\textheight]{iccv2023AuthorKit/figure/mmreact-unfolded-4.pdf}
% \vspace{-30mm}
% \caption{Unfolded multimodal reasoning and action steps for the input image, and the user question is ``Where is the coffee pot in the second image?'' % \url{https://microsoft-my.sharepoint.com/:p:/g/personal/keli_microsoft_com1/EYmEmA2AKJFCoUt2vZtY_1EB5zPERmgT7zU-kR7EMls-0g?e=ECYFyu}
% 	}
% \label{fig:mmreact-unfolded-4}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=.85\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme-mmreact-cot2.pdf}
% \vspace{-14mm}
% \caption{Illustration of chain-of-thoughts 
% 	}
% \label{fig:palme-cot-2}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=.85\textwidth]{iccv2023AuthorKit/figure/palme_compare/palme-mmreact-cot.pdf}
% \vspace{-18mm}
% \caption{Illustration of chain-of-thoughts 
% 	}
% \label{fig:palme-cot}
% \end{figure*}
